Relations between the Worldline Quantum Field Theory and scattering amplitudes for particles with spin

The Worldline Quantum Field Theory (WQFT) has proven to be an efficient tool for calculating observables in gravitational wave physics. In contrast to other QFT-based techniques in the realm of gravitational wave physics, it makes the classical limit very apparent. However, a natural question remains: How does it relate to ordinary quantum field theories that we know from particle physics? This question will be addressed by extending existing approaches to a description including spin. Furthermore, it will be explicitly shown that the WQFT can retain quantum contributions by summing up infinite towers of worldline loops.

==> chapters/Selbststa__ndigkeitserkla__rung.tex <==
\section*{Selbstständigkeitserklärung}
\noindent Ich erkläre hiermit, dass ich die vorliegende Arbeit selbstständig verfasst und noch nicht für andere Prüfungen eingereicht habe. Sämtliche Quellen einschließlich Internetquellen, die unverändert oder abgewandelt wiedergegeben werden, insbesondere Quellen für Texte, Grafiken, Tabellen und Bilder, sind als solche kenntlich gemacht. Mir ist bekannt, dass bei Verstößen gegen diese Grundsätze ein Verfahren wegen Täuschungsversuchs bzw. Täuschung eingeleitet wird.\\ \ \\
Berlin, den 30.09.2022   ........................................................................................................
